Land Cover Changes Cause Increased Losses during Photosynthetic Extremes

Human-induced carbon dioxide (CO2) emissions, primarily from fossil fuel combustion and changes in land use and land cover (LULCC), are a key contributor to climate change. As the climate warms, extreme events such as heatwaves, droughts, and wildfires have become more frequent and are projected to intensify throughout the 21st century. These escalating extremes are likely to further disrupt vegetation productivity, known as gross primary production (GPP), and reduce the ecosystem's capacity to absorb carbon. In this study, we employ a global Earth system model to assess how (a) CO2 emissions alone and (b) CO2 combined with LULCC influence the severity, frequency, and duration of GPP extremes. Our results show that negative GPP extremes periods of unexpectedly low carbon uptake are increasing more rapidly than positive extremes, especially under LULCC scenarios. The primary climate factor driving these extremes is soil moisture variability, which is influenced by fluctuations in both precipitation and temperature. The delayed responses of GPP to different climate drivers depend on the specific driver and geographical region. Overall, the highest incidence of GPP extremes arises from the combined influence of water stress, temperature anomalies, and fire-related disturbances.

==> figure_gpp_regions_wo_iav.tex <==
 \begin{figure}
 \centering
 \includegraphics[trim = {0.1cm 0.1cm 0.1cm .85cm},clip,width=0.95\columnwidth]{figures/diff/gpp_regions_wo_iav.pdf}
 \caption{The IAV of GPP for the simulation without LULCC. The IAV is calculated from 1850 as the base year to 25~year increments, as shown in $x$-axis. This figure shows the IAV of GPP at four randomly selected grid cells (Table~\ref{t:locations_of_regions}) in each region A, B, C, and D.}
\label{f:gpp_regions_wo_iav}
\end{figure}


==> figure_gpp_regions_wo_trend.tex <==
\begin{figure}
 \centering
 \includegraphics[trim = {0.1cm 0.1cm 0.1cm .85cm},clip,width=0.95\columnwidth]{figures/diff/gpp_regions_wo_trend.pdf}
 \caption{Trends in GPP for the simulation without LULCC. The trends are calculated from 1850 as the base year to 25~year increments, as shown in $x$-axis. This figure shows the trends in GPP at four randomly selected grid cells (Table~\ref{t:locations_of_regions}) in each region A, B, C, and D.}
\label{f:gpp_regions_wo_trend}
\end{figure}


==> figure_prcp_regions_wo_trend.tex <==
\begin{figure}
 \centering
 \includegraphics[trim = {0.1cm 0.1cm 0.1cm .85cm},clip,width=0.95\columnwidth]{figures/diff/prcp_regions_wo_trend.pdf}
 \caption{Trends in precipitation for the simulation without LULCC. The trends are calculated from 1850 as the base year to 25~year increments, as shown in $x$-axis. This figure shows the trends in precipitation at four randomly selected grid cells (Table~\ref{t:locations_of_regions}) in each region A, B, C, and D. }
\label{f:prcp_regions_wo_trend}
\end{figure}


==> figure_sm_regions_wo_trend.tex <==
\begin{figure}
 \centering
 \includegraphics[trim = {0.1cm 0.1cm 0.1cm .85cm},clip,width=0.95\columnwidth]{figures/diff/sm_regions_wo_trend.pdf}
 \caption{Trends in soil moisture for the simulation without LULCC. The trends are calculated from 1850 as the base year to 25~year increments, as shown in $x$-axis. This figure shows the trends in soil moisture at four randomly selected grid cells (Table~\ref{t:locations_of_regions}) in each region A, B, C, and D.}
\label{f:sm_regions_wo_trend}
\end{figure}

